URDF-Anything: Constructing Articulated Objects with 3D Multimodal Language Model

Constructing accurate digital twins of articulated objects is essential for robotic simulation training and embodied AI world model building, yet historically requires painstaking manual modeling or multi-stage pipelines. In this work, we propose \textbf{URDF-Anything}, an end-to-end automatic reconstruction framework based on a 3D multimodal large language model (MLLM). URDF-Anything utilizes an autoregressive prediction framework based on point-cloud and text multimodal input to jointly optimize geometric segmentation and kinematic parameter prediction. It implements a specialized $[SEG]$ token mechanism that interacts directly with point cloud features, enabling fine-grained part-level segmentation while maintaining consistency with the kinematic parameter predictions. Experiments on both simulated and real-world datasets demonstrate that our method significantly outperforms existing approaches regarding geometric segmentation (mIoU 17\% improvement), kinematic parameter prediction (average error reduction of 29\%), and physical executability (surpassing baselines by 50\%). Notably, our method exhibits excellent generalization ability, performing well even on objects outside the training set. This work provides an efficient solution for constructing digital twins for robotic simulation, significantly enhancing the sim-to-real transfer capability.

==> sec/0_abstract.tex <==
  % The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
  % both the left- and right-hand margins. Use 10~point type, with a vertical
  % spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
  % bold, and in point size 12. Two line spaces precede the abstract. The abstract
  % must be limited to one paragraph.

% 构建精确的铰接物体数字孪生对机器人仿真训练和具身智能世界模型构建至关重要。然而，传统方法依赖人工建模或简化几何表示，难以兼顾复杂部件的几何保真度与运动参数推理的准确性。

% 针对这一挑战，我们提出了URDF-Anything，一种基于多模态大语言模型（MLLM）的端到端重建框架。URDF-Anything使用基于点云和文本多模态输入的自回归预测框架，联合优化几何分割与运动参数预测，实现形状与运动特性的统一建模；在此基础上，进一步引入动态分割机制，利用可学习的[SEG]标记与点云特征交互，实现部件级精确分割。

% 在仿真环境和真实场景数据上的实验表明，我们的方法在部件分割、关节参数预测及物理可执行性上均显著优于现有方法。特别地，我们的方法对训练集外物体仍表现出色，展现出卓越的泛化能力。这项工作为机器人仿真提供了高效的数字孪生构建方案，显著提升了模拟到现实的迁移能力。

\begin{abstract}

Constructing accurate digital twins of articulated objects is essential for robotic simulation training and embodied AI world model building, yet historically requires painstaking manual modeling or multi-stage pipelines. In this work, we propose \textbf{URDF-Anything}, an end-to-end automatic reconstruction framework based on a 3D multimodal large language model (MLLM). URDF-Anything utilizes an autoregressive prediction framework based on point-cloud and text multimodal input to jointly optimize geometric segmentation and kinematic parameter prediction. It implements a specialized $[SEG]$ token mechanism that interacts directly with point cloud features, enabling fine-grained part-level segmentation while maintaining consistency with the kinematic parameter predictions.
Experiments on both simulated and real-world datasets demonstrate that our method significantly outperforms existing approaches regarding geometric segmentation (mIoU 17\% improvement), kinematic parameter prediction (average error reduction of 29\%), and physical executability (surpassing baselines by 50\%). Notably, our method exhibits excellent generalization ability, performing well even on objects outside the training set. This work provides an efficient solution for constructing digital twins for robotic simulation, significantly enhancing the sim-to-real transfer capability.

\end{abstract}

% 1. 任务是什么？ 用 3d llm 做 urdf 任务
% 2. 当前前人方法没有解决，没有解决好的是什么（概括解决前任技术的缺点，重点是前人没有实现好的效果，从效果角度）， 举例说明任务的重要性（社区数据集）=⇒ 任务需要做什么，但是前人方法没有做到什么
% a. 社区铰接物体数据集（更方便的获取）
% b. 3d llm做urdf任务
% c. 框架创新（待定），效果好（待定）
% d. 其他任务都是mesh retrival，我们是mesh generation
% e. 前人未能解决的是铰接物体的全参数预测

% - 第一句话：urdf 数据集在xxx领域很重要
% - 第二句话：前人要么是传统方法（概括名字），要么是mesh retrival，要么是digital consuin，忽略了mesh generation
% - 第三句话：为了实现真正意义的digital twin
% - 第四句话：因此，我们提出了 Urdf-Anything 方法，支持单张图片和多张图片输入，生成 urdf 文件
% - 第五句话：任务特征分析， specifically，为了生成urdf，将分割引入3d llm
% - 第六句话：提出技术细节
% - 第七句话：我们最终实现了高质量的urdf生成


==> sec/1_introduction.tex <==
\section{Introduction}

% Constructing high-fidelity digital twins is essential for accurately simulating real-world physical dynamics and agent–object interactions—an indispensable foundation for robot learning. However, populating these interactive virtual environments requires precise digital representations of their components, especially articulated objects (doors, drawers, tools, furniture) with their complex internal structures and diverse degrees of freedom, which typically demands painstaking manual modeling, specialized expertise, and extensive development time. Automating the reconstruction of these objects into fully functional, high-fidelity digital twins (for example, in URDF format) not only alleviates this laborious effort but also offers an efficient pathway to enrich virtual worlds and enable robust simulation-to-real transfer in robotic training.


Constructing high-fidelity digital twins is essential for accurately simulating real-world physical dynamics and complex interactions across numerous fields. These include core applications in robotic simulation and training\cite{baratta2024digital,li2025digital} as well as expanding domains like autonomous driving\cite{hossain2023neweramobilityexploring,Zhou2024ReviewOD,Kizilirmak2023DigitalTA} and interactive virtual/augmented reality environments\cite{lee2008recent,wang2020vr,kim2025metaobjectsinteractivemultisensoryvirtual}. 
However, populating these interactive virtual environments requires precise digital representations of their components, especially articulated objects (doors, drawers, scissors) with their complex internal structures and diverse degrees of freedom, which typically demands painstaking manual modeling, and extensive development time. 
Automating the reconstruction of these objects into fully functional, high-fidelity digital twins (for example, in URDF format) not only alleviates this laborious effort but also offers an efficient pathway to enrich virtual worlds and enable robust simulation-to-real transfer in robotic training.

However, automatically reconstructing articulated objects from visual observations presents significant challenges. Unlike rigid objects, articulated objects consist of multiple parts connected by joints, introducing complexities related to inferring both the geometry of individual links and the kinematic parameters (type, origin, axis, limits) governing their motion. Prior efforts reconstruct articulated objects by composing multiple models into a sophisticated pipeline and either rely on a given mesh assets library or involve a separate part segmentation stage~\cite {mandi2024real2code,le2025articulateanything}.

In this paper, we explore an end-to-end approach for generating functional URDF models directly from visual input;
we propose \textbf{URDF-Anything}, which leverages 3D Multimodal Large Language Models (MLLMs) to jointly interpret object geometry and semantic attributes, infer kinematic structure, and automatically produce high-fidelity URDF descriptions (Figure~\ref{fig:overall-structure} illustrates the overall pipeline). 
A 3D MLLM is uniquely suited for this task, as it can natively handle multimodal input (visual features and text instructions), encodes powerful priors on 3D shapes from large-scale pretraining, and directly understands spatial relationships to output precise coordinates. These capabilities make it ideal for predicting detailed kinematic parameters and generalizing to unseen objects. In addition, we introduce a novel dynamic $[SEG]$ token mechanism~\cite{lai2024lisa} within the MLLM’s autoregressive generation, which enables simultaneous prediction of the symbolic articulated structure (link names, joint parameters) and emission of explicit segmentation signals that guide geometric segmentation of object parts from point-cloud features via cross-attention. This tight coupling between symbolic output and geometric segmentation, combined with end-to-end training, ensures full consistency between predicted kinematics and reconstructed geometry, and enables an end-to-end approach for reconstructing articulated objects.

Experimental evaluation on the PartNet-Mobility dataset~\cite{mo2018partnetlargescalebenchmarkfinegrained}, including both in-distribution and challenging out-of-distribution objects, demonstrates the superior performance of URDF-Anything compared to existing methods. Quantitatively, for part-level geometric segmentation,we achieve higher mIoU on OOD instances (0.62) compared to the best baseline (0.51), and a much higher Count Accuracy (0.97), surpassing the best baseline (0.84) by over 15 points. 
In joint parameter prediction, our method consistently achieves significantly lower errors across all object categories compared to baselines, outperforming them by a considerable margin, particularly on complex and OOD objects. Crucially, the physical executability rate of our generated URDF models is substantially higher than baselines(50\% improvement), enabling more robust simulation for complex and OOD objects. These comprehensive results highlight the effectiveness and strong generalization capability of our end-to-end MLLM framework for automated articulated object reconstruction.


% Our main contributions are summarized as follows:
% \begin{itemize}
%     \item We propose \textbf{URDF-Anything}, a novel framework leveraging a 3D MLLM for articulated object reconstruction from visual input to URDF.
%     \item We introduce a novel dynamic $[SEG]$ token mechanism that enables the MLLM to jointly generate structured kinematic parameters and perform part-level geometric segmentation via direct token-feature interaction.
%     \item Our method achieves state-of-the-art performance on geometric segmentation, kinematic parameter prediction, and physical executability on the PartNet-Mobility dataset, demonstrating superior generalization to complex and unseen objects.
% \end{itemize}

==> sec/2_related_works.tex <==
\section{Related Work}

% 记得写中文大纲，作为注释，主要是你的写作逻辑，写作思路 
% # articulated object modeling
% 1. 从真实世界重建铰接物体结构：已经取得显著进展
%。  1.传统方法：通过few-shot交互
%       1.paper
%           1.Ditto: Building Digital Twins of Articulated Objects from Interactio
dataset=splart-pms
obj=103031-CoffeeMachine
timestamp=$(date -u +%Y-%m-%dT%H:%M:%SZ)
ns-train splart \
    --output-dir model_ckpts/$dataset \
    --experiment-name $obj/$timestamp \
    --vis wandb \
    --data datasets/splart/$dataset/$obj \
    --max-num-iterations 25000 \
    --pipeline.model.num-random 999999 \
    --pipeline.model.random-scale 1.3%           2.Sim2Real2: Actively Building Explicit Physics Model for Precise Articulated Object Manipulation
%           3.Sim2Real2 : Actively Building Explicit Physics Model for Precise Articulated Object Manipulation
%           4.Structure from Action: Learning Interactions for 3D Articulated Object Structure Discovery
%       2.缺点：获取更困难，缺少互联网数据
%。  2.基于图片，mesh retrieval 方法
%。     1.paper
%          1.URDFormer: A Pipeline for Constructing  Articulated Simulation Environments from  Real-World Images
%。         2.ARTICULATE-ANYTHING:  AUTOMATIC MODELING OF ARTICULATED OBJECTS  VIA A VISION-LANGUAGE FOUNDATION MODEL
%。         3.Automated Creation of Digital Cousins for Robust Policy Learning
%。     2.缺点：灵活性不够，泛化性差，重建不够准确
%    3.基于图片，由点云进行分割、重建
%。     1.paper
%          1.BUILDING INTERACTABLE REPLICAS OF COMPLEX  ARTICULATED OBJECTS VIA GAUSSIAN SPLATTING
%          2. Real2Code: Reconstruct Articulated Objects via Code Generation
%       2.缺点：需要multi-view图片。未生成urdf表达形式
% 2.我们：基于单张图片，mesh generation

%#LLMs for 3D Tasks
%1. papers
%   1.ShapeLLM: Universal 3D Object Understanding for Embodied Interaction
%   2.MeshGPT: Generating Triangle Meshes with Decoder-Only Transformers
%。  3.LLaVA-3D: A Simple yet Effective Pathway to Empowering LMMs with 3D-awareness
\textbf{LLMs for 3D Tasks.}
Recent years have seen significant progress in applying Large Multimodal Models (LMMs) to 3D understanding and interaction tasks~\cite{chen2024ll3da,chen2024spatialvlm,deng2024can,qi2024gpt4point,chen2024grounded,xu2025pointllm,yuan2024visual,deng20253d,yang2023lidar}. These models leverage multimodal inputs (such as point clouds or images, combined with language) for 3D spatial reasoning, perception, and structured output generation. Relevant advancements include the development of 3D MLLM backbones like ShapeLLM~\cite{qi2024shapellmuniversal3dobject}, capable of handling point cloud-language interaction and demonstrating strong 3D understanding. Other works have explored language-guided 3D segmentation~\cite{he2024segpointsegmentpointcloud}, open-world 3D understanding~\cite{zhu2023pointclipv2promptingclip}, and tasks requiring precise 3D spatial understanding from visual input~\cite{yang2025llmi3dmllmbased3dperception}. While these models demonstrate powerful capabilities in general 3D perception and generating text or segmentation masks, they do not typically address the complex, coupled task of jointly inferring detailed link geometry and precise kinematic parameters for articulated objects. Our work builds upon these advancements in 3D LMMs and their capabilities for spatial reasoning and multimodal generation, specifically applying them to the challenging task of articulated object reconstruction.

\textbf{Articulated object modeling.}
Research on the reconstruction and modeling of articulated objects specifically for robotic manipulation is a related but distinct field. Physics-based interactive methods~\cite{lv2022sagcisystemsampleefficientgeneralizablecompositional, hsu2024kinscenemodelbasedmobilemanipulation, ma2023sim2real2activelybuildingexplicit} utilize interaction in simulation or the real world to refine or build models, demonstrating high accuracy with sufficient interaction but often requiring initial models, struggling with robust passive reconstruction (without interaction), or limited adaptation to novel geometries without extensive interaction data. 
Automation methods ~\cite{le2025articulateanything,mandi2024real2code} leveraging visual-language models  automate digital twin creation, using techniques such as VLM-to-code generation, iterative refinement, mesh retrieval~\cite{le2025articulateanything}, or abstracting parts as OBBs with LLM parameter prediction~\cite{mandi2024real2code}. However, these methods can be limited by constraints such as reliance on asset databases, brittleness in iterative processes, or loss of geometric detail and potential parameter inaccuracy from using simplified representations like OBBs. ~\cite{chen2024urdformer} focuses on generating articulated simulation scenes from images, which is related but distinct from accurate individual object parameter reconstruction and doesn't guarantee parameter accuracy or physics fidelity for novel objects.
Other works~\cite{liu2025artgs,liu2023paris,lei2023gartgaussianarticulatedtemplate,ma2024magsreconstructingsimulatingdynamic,wu2025reartgsreconstructinggeneratingarticulated} explore novel representations like 3D Gaussians for reconstruction or focus on detection of specific features~\cite{sun2023opdmultiopenabledetectionmultiple}, addressing sub-problems rather than the complete, end-to-end geometry and kinematics inference pipeline needed for a functional URDF. Our work contributes to the field of automated articulated object modeling by proposing a novel end-to-end framework that leverages the capabilities of 3D Large Multimodal Models for robust reconstruction from visual input.

==> sec/3_method.tex <==
\section{Method}
\label{gen_inst}


URDF-Anything is an end-to-end framework for reconstructing articulated objects from visual observations into URDF-formatted digital twins. The pipeline consists of three main stages: (1) Input Representation, where we generate dense 3D point clouds from single or multi-view RGB images, in Sec\ref{Input Representation} ; (2) Multimodal Articulation Parsing, where a 3D Multimodal Large Language Model (MLLM) jointly predicts part segmentation and kinematic parameters, in Sec\ref{MLLM} ; and (3) Mesh Conversion, where segmented point clouds are converted into meshes for simulation, in Sec\ref{mesh_conv}. The key innovation lies in the integration of geometric and semantic features through a dynamic $[SEG]$ token mechanism, enabling precise part-level segmentation and joint parameter prediction in a unified framework.

\subsection{Task Definition}
\label{headings}

To ensure compatibility with standard 3D simulators (e.g., MuJoCo, PyBullet), we represent articulated objects as URDF (Unified Robot Description Format) models. A URDF structure defines an object as a hierarchical tree composed of:

\textbf{Links}: Rigid components representing object parts (e.g., a cabinet’s door, drawer, or base). Each link contains geometric (mesh) and inertial properties.

\textbf{Joints}: Connections between links that specify kinematic constraints. Each joint includes: 
\begin{itemize}[topsep=0pt, partopsep=0pt, itemsep=0pt, parsep=0pt]
    \item Type: Prismatic, revolute, continuous, floating, planar or fixed.
    \item Parent/Child: Links connected by the joint.
    \item Origin : 3D position $(x,y,z)\in \mathbb{R}^3$ and orientation $(r, p, y)\in \mathbb{R}^3$ relative to the parent link.
    \item Axis: Normalized 3D vector defining the motion direction (e.g., $[0,1,0]$ for vertical sliding).
    \item Limit: Defines the range of motion for prismatic, revolute and planar joints.
\end{itemize}
Our objective is to automatically infer these URDF components—specifically, the mesh for each link, the type, origin, parent, child, and axis for each joint—from visual input of the articulated object.

\begin{figure*}[t]
\label{fig:overall-structure}
\centering
\includegraphics[page=1,width=1.0\textwidth]{figure/nips_overall2.pdf}
\caption{Overview of the URDF-Anything Framework. The pipeline takes a 3D point cloud (from image) and a structured language instruction as input. The 3D MLLM(fine-tuned with LoRA) autoregressively generates symbolic output (kinematic parameters) and $[SEG]$ tokens. The embeddings corresponding to the generated $[SEG]$ tokens then interact with the point cloud features via a 3D Decoder to perform fine-grained geometric segmentation of the point cloud into individual links. Finally, the jointly predicted kinematic parameters and the segmented geometry are integrated into a functional URDF file, resulting in a complete articulated 3D model ready for physics simulation.}
\label{fig:overall-structure}
% \vspace{-2em}
\end{figure*}


\subsection{Input Representation} \label{Input Representation}
The initial step of our pipeline is to transform the raw visual observation of an articulated object into a 3D representation suitable for structural parsing. Real-world observations can vary significantly, sometimes providing multiple viewpoints of the object and other times offering only a single view. Accordingly, our point cloud acquisition strategy adapts to the input modality:  

\textbf{Multi-view Input:} When multiple RGB images from different viewpoints are available , we leverage  DUSt3R\cite{wang2024dust3rgeometric3dvision} to generate a dense 3D point cloud $P_{obj}$. DUSt3R excels at establishing dense 2D-to-3D correspondences and reconstructing accurate 3D geometry from multiple views.  

\textbf{Single-view Input:} For the more challenging single-view scenario, we utilize a generative approach LGM\cite{tang2024lgmlargemultiviewgaussian}. We first employ a pre-trained diffusion model to synthesize consistent multi-view images. Subsequently, we reconstruct the 3D geometry from these synthesized views, which can be represented as a 3D Gaussian Splatting model or converted into a point cloud $P_{obj}$.  

Regardless of the input type (single or multi-view), the output of this stage is a dense point cloud $P_{obj} \in \mathbb{R}^{N \times 6}$ representing the entire articulated object. It is crucial to note that this initial point cloud is a monolithic representation; it captures the overall geometry but does not inherently differentiate or segment the object into its individual links or sub-components. This whole-object point cloud $P_{obj}$ serves as the primary geometric input for the subsequent multimodal articulation parsing stage. More details about this section are reported in Appendix \ref{pc_details}.

% \subsection{3D MLLM Backbone}
% We adopt ShapeLLM  as our backbone, which combines a ReCon++ point cloud encoder with a LLaMA-2 language model. ShapeLLM has demonstrated the ability to perform 3D visual grounding and output structured 3D information, such as 3d bounding box coordinates. This pre-existing capability for generating precise 3D spatial outputs is particularly beneficial for our task of predicting joint parameters, which inherently involve 3D locations (origin, axis) and orientations (origin). This unified architecture offers two advantages: (1) Open-world generalization:  The 3D MLLM's geometric understanding capability, enhanced by large-scale 3D-language pretraining, enables robust reasoning about both seen and unseen object categories. (2) Structured output capability: The MLLM inherently supports generating JSON-formatted outputs of arbitrary length and complexity, enabling flexible representation of joint hierarchies and part relationships.

% \textbf{3D MLLM:} The input point cloud $P_{obj}$ is encoded by a 3D encoder to extract dense geometric features $F_{pc} \in \mathbb{R}^{M \times d_{pc}}$, where $M$ is the number of points (potentially downsampled) and $d_{pc}$ is the feature dimension. Simultaneously, natural language instructions are provided to guide the parsing process. We employ a structured instruction template (illustrated in Figure~1) that explicitly incorporates the geometric features and prompts the model for specific URDF information. Here, the special <point> token serves as a placeholder for the point cloud features $F_{pc}$. The textual part of the instruction, $X_{txt}$, is processed by the LLM's standard word embedding layer to yield text embeddings $F_{txt} \in \mathbb{R}^{L \times d_{txt}}$, where $L$ is the number of tokens and $d_{txt}$ is the embedding dimension. These multimodal features ($F_{pc}$ and $F_{txt}$) are integrated and processed by the LLM's layers.  This core multimodal processing and output generation can be formally represented as:
% $$ Y_{output} = \text{MLLM}(F_{pc}, F_{txt}) $$
% The output text $Y_{output}$ would include $N$ [SEG] tokens, where $N$ is the number of objects part. We will discuss [SEG]-related content next.

% \textbf{Dynamic [SEG] Token Mechanism:} While MLLMs like ShapeLLM excel at processing multimodal inputs and generating structured textual outputs, they are not inherently equipped for generating dense, per-point predictions required for geometric segmentation. Our task necessitates not only predicting the symbolic URDF structure and parameters but also precisely segmenting the corresponding point cloud geometry for each link.

% To achieve this joint objective, inspired by LISA [27], we extend the vocabulary with a specialized [SEG] token. The MLLM is trained to autoregressively generate a structured JSON output sequence that contains the predicted joint parameters (type, origin, axis, parent, child) alongside descriptions of the links. Crucially, each link description in the output is associated with a [SEG] token (e.g., "link\_0": "base\_cabinet[SEG]", "link\_1": "drawer[SEG]"). This means the MLLM simultaneously predicts the symbolic representation of the articulated structure and places markers ([SEG]) indicating the geometry corresponding to each part needs to be identified.

% % These multimodal features are concatenated [F_pc;F_txt]  and fed into the MLLM, which generates output sequences containing alternating [SEG] tokens and textual descriptions. For each generated [SEG] token, we extract its final hidden state representation h_seg = MLLM([F_pc;F_txt])[SEG] ∈ ℝ^d that encapsulates both semantic meaning and spatial relationships learned through the model's attention mechanisms. This token representation then interacts with the original point cloud features through a cross-attention operation Q = MLP(h_seg) ∈ ℝ^{d×d'}, K,V = Proj(F_pc) ∈ ℝ^{N×d'}, yielding segmentation probabilities y_mask = Softmax(QK^⊤/√d')V ∈ ℝ^N that precisely associate 3D points with their corresponding object parts. The attention mechanism naturally handles varying point densities by computing adaptive affinity scores between each point and the [SEG] token, then aggregating features weighted by their part relevance. 


% \textbf{Geometric Segmentation Guided by Dynamic Tokens:}
% Upon generating the output sequence $Y_{output}$, which includes link names paired with $[SEG]$ tokens, we initiate the geometric segmentation process. For each instance of a [SEG] token appearing in the output, we utilize its corresponding hidden state from the final layer of the LLM, $h_{seg} \in \mathbb{R}^{d_{emb}}$. To enrich the query signal for segmentation, we concatenate $h_{seg}$ with the hidden state of the preceding token in the output sequence, which represents the predicted part category (e.g., "base\_cabinet"), denoted as $h_{category} \in \mathbb{R}^{d_{emb}}$. The combined feature vector $h_{combined} \in \mathbb{R}^{2 \times d_{emb}}$ is computed as:
% $$ h_{combined} = [h_{seg} ; h_{category}] $$
% This fused representation leverages both the segmentation signal from `[SEG]` and the semantic information from the predicted part name.

% To enable interaction between this combined token feature and the dense point cloud features $F_{pc}$, we project both into a common embedding space of dimension $d_{attn}$:
% $$ H_{query} = \text{MLP}_{query}(h_{combined}) \in \mathbb{R}^{d_{attn}} $$
% $$ F'_{pc} = \text{MLP}_{pc}(F_{pc}) \in \mathbb{R}^{M \times d_{attn}} $$
% where $\text{MLP}_{query}$ and $\text{MLP}_{pc}$ are learned linear projection layers (MLPs).

% The projected combined token feature $H_{query}$ serves as the query in a cross-attention mechanism that attends over the projected point cloud features $F'_{pc}$ (serving as Key and Value):
% $$ y_{mask} = \text{CrossAttn}(Q=H_{query}, K=F'_{pc}, V=F'_{pc}) $$
% The output $y_{mask} \in \mathbb{R}^{M}$ provides a vector of per-point scores (logits) indicating the likelihood of each point in the original point cloud $P_{obj}$ belonging to the specific part associated with the [SEG] token. By applying a sigmoid function and a threshold to $y_{mask}$, we obtain the binary segmentation mask for the link. This process is repeated for every `[SEG]` token in the output sequence, yielding a complete set of segmentation masks for all predicted parts.


% \textbf{Hierarchical Segmentation:} % This section is now integrated above
% The token interacts with point cloud features through:
% $$y_{mask}=CrossAttn(Q=Hseg,K=Fpc,V=Fpc)$$



% \jy{revision of 3.3====}

\subsection{Articulation Parsing with 3D MLLM} \label{MLLM}
We adopt ShapeLLM~\cite{qi2024shapellmuniversal3dobject}, a recent 3D MLLM, as our backbone, which combines a point cloud encoder\cite{qi2023contrastreconstructcontrastive3d} with a large language model\cite{touvron2023llamaopenefficientfoundation}. ShapeLLM has demonstrated the ability to perform 3D visual grounding and output structured 3D information, such as 3D bounding-box coordinates. 
This pre-existing capability is particularly beneficial for our task of predicting joint parameters, which inherently involve 3D locations (origin, axis) and orientations (origin). 
This unified architecture offers two advantages: (1) Open-world generalization:  The 3D MLLM's geometric understanding capability, enhanced by large-scale 3D-language pretraining, enables robust reasoning about both seen and unseen object categories. (2) Structured output capability: The MLLM inherently supports generating JSON-formatted outputs of arbitrary length and complexity, enabling flexible representation of joint hierarchies and part relationships.

\textbf{Input:} The input point cloud $P_{obj}$ is encoded by a 3D encoder to extract dense geometric features $F_{pc} \in \mathbb{R}^{M \times d_{pc}}$, where $M$ is the number of points (potentially downsampled) and $d_{pc}$ is the feature dimension. Simultaneously, natural language instructions are provided to guide the parsing process. We employ a structured instruction template that explicitly incorporates the geometric features and prompts the model for specific URDF information. The textual part of the instruction, $X_{txt}$, is processed by the LLM's standard word embedding layer to yield text embeddings $F_{txt} \in \mathbb{R}^{L \times d_{txt}}$, where $L$ is the number of tokens and $d_{txt}$ is the embedding dimension. These multimodal features ($F_{pc}$ and $F_{txt}$) are integrated and processed by the LLM's layers.  This core multimodal processing and output generation can be formally represented as:
$$ Y_{output} = \text{MLLM}(F_{pc}, F_{txt}) $$


\textbf{Output:} While 3D MLLMs excel at processing multimodal inputs and generating structured textual outputs, they are not inherently equipped to generate dense, per-point predictions required for geometric segmentation. Our task necessitates not only predicting the symbolic URDF structure and parameters but also precisely segmenting the corresponding point cloud geometry for each link.
Inspired by LISA\cite{lai2024lisa}, we extend the vocabulary with a special token $[SEG]$ to achieve this joint objective. The MLLM is trained to autoregressively generate a structured JSON output sequence that contains the predicted joint parameters alongside descriptions of the links. Crucially, each link description in the output is associated with a $[SEG]$ token (e.g., "link\_0": "base\_cabinet$[SEG]$", "link\_1": "drawer$[SEG]$"). This means the MLLM simultaneously predicts the symbolic representation of the articulated structure and places markers ($[SEG]$) indicating the geometry corresponding to each part needs to be identified. More details are reported in Appendix \ref{instruction_details}.

\subsection{Geometric Segmentation from Special-Token Mechanism} \label{sec:geometric_segmentation}

% These multimodal features are concatenated [F_pc;F_txt]  and fed into the MLLM, which generates output sequences containing alternating [SEG] tokens and textual descriptions. For each generated [SEG] token, we extract its final hidden state representation h_seg = MLLM([F_pc;F_txt])[SEG] ∈ ℝ^d that encapsulates both semantic meaning and spatial relationships learned through the model's attention mechanisms. This token representation then interacts with the original point cloud features through a cross-attention operation Q = MLP(h_seg) ∈ ℝ^{d×d'}, K,V = Proj(F_pc) ∈ ℝ^{N×d'}, yielding segmentation probabilities y_mask = Softmax(QK^⊤/√d')V ∈ ℝ^N that precisely associate 3D points with their corresponding object parts. The attention mechanism naturally handles varying point densities by computing adaptive affinity scores between each point and the [SEG] token, then aggregating features weighted by their part relevance. 


Geometric segmentation is performed for each object part indicated by a $[SEG]$ token in the MLLM's output sequence $Y_{output}$. For each generated $[SEG]$ token, we leverage its final hidden state $h_{seg}$, combined with the preceding part category token's state $h_{category}$ to form a fused token representation $h_{combined} = [h_{seg} ; h_{category}]$. This representation is then used as the query $$H_{query} = \text{MLP}_{query}(h_{combined})$$ in a cross-attention mechanism. 
Another point feature $S_{pc}$ is generated from 3D backbone $S_{pc} = F_{enc}(P_{obj})$. Then a mechanism attends over the projected point cloud features $F'_{pc} = \text{MLP}_{pc}(S_{pc})$, effectively computing per-point scores $$y_{mask} = \text{CrossAttn}(Q=H_{query}, K=F'_{pc}, V=F'_{pc})$$ indicating the likelihood of each point belonging to the part. These scores $y_{mask}$ are converted into a binary segmentation mask for the corresponding link via a sigmoid and threshold. This process is repeated for every $[SEG]$ token, yielding masks for all predicted parts.

% \textbf{Hierarchical Segmentation:} % This section is now integrated above
% The token interacts with point cloud features through:
% $$y_{mask}=CrossAttn(Q=Hseg,K=Fpc,V=Fpc)$$

\subsection{Mesh Conversion and URDF File Generation} \label{mesh_conv}
The final stage of our pipeline consolidates the reconstructed geometry and kinematics into a standard URDF XML file, ready for direct use in physics simulators. Segmented point clouds for each link, obtained from the geometric segmentation process (Section~\ref{sec:geometric_segmentation}), are converted into 3D mesh representations (e.g., OBJ format) using point-to-mesh conversion method\cite{1056714,817351}. Simultaneously, the MLLM's structured JSON output provides the complete kinematic structure, including joint types, parent/child relationships, origins, and axis. We parse this JSON and assemble the final URDF XML file, where each link references its generated mesh and joint elements are populated with the predicted parameters. The resulting URDF model can be directly imported into standard physics simulators (e.g., MuJoCo~\cite{todorov2012mujoco}, Sapiens~\cite{khirodkar2024sapiens}). A complete example of a generated URDF file for a sample object instance is provided in Figure\ref{fig:urdf_appendix}.

\subsection{Model Training}
The URDF-Anything model is trained end-to-end to jointly generate the structured URDF parameters and predict accurate part-level segmentation masks from the point cloud. The overall training objective $L$ is a weighted sum of the language modeling loss $L_{text}$ and the segmentation loss $L_{seg}$: $$ L = \lambda_{text} L_{text} + \lambda_{seg} \sum_{i=1}^{N} L_{i, seg} $$ 
where $\lambda_{lm}$ and $\lambda_{seg}$ are hyperparameters balancing the contribution of each loss, and $N$ is the num of object parts. The segmentation loss uses a combination of binary cross-entropy (BCE) loss and Dice loss (DICE). For a given part associated with a $[SEG]$ token, let $M_{gt} \in \{0, 1\}^M$ be the ground truth binary mask for that part. The segmentation loss for this part is: 
$$ L_{seg} = \lambda_{bce} \text{BCE}(\hat{M}, M_{gt}) + \lambda_{dice} \text{DICE}(\hat{M}, M_{gt}) $$ 
where $\lambda_{bce}$ and $\lambda_{dice}$ are hyperparameters weighting the BCE and DICE components. 


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=1 \linewidth]{figure/nips_workflow.pdf}
%     \caption{Step-by-Step Reconstruction from Real-World Image to Functional URDF.
%     \vspace{-2mm}
%     }
%     \label{fig:workflow}
% \end{figure}

==> sec/4_experiments.tex <==
\section{Experiments} \label{Exp}

\textbf{Implementation Details:} 
We employ ShapeLLM~\cite{qi2024shapellmuniversal3dobject} as our 3D MLLM backbone, with ShapeLLM-7B-general-v1.0 checkpoint as the default settings. For the 3D backbone, We use Uni3D~\cite{zhou2023uni3d} to extract dense geometric features. We adopt one NVIDIA 80G A800 GPU for training. We employ LoRA~\cite{hu2021loralowrankadaptationlarge} for efficient fine-tuning, with the rank of LoRA set to 8 by default. We use AdamW optimizer~\cite{loshchilov2019decoupledweightdecayregularization} with the learning rate and weight decay set to 0.0003 and 0, respectively. We use the cosine learning rate scheduler, with the warm-up iteration ratio set to 0.03. The batch size per device is set to 2, and the gradient accumulation step is set to 10.


\textbf{Dataset:} 
We train and evaluate our framework on the PartNet-Mobility dataset~\cite{mo2018partnetlargescalebenchmarkfinegrained}, a large collection of 3D articulated objects with URDF annotations. Since our method utilizes image input, we generated visual data by rendering multi-view and single-view RGB images from the dataset's 3D models within a simulation environment. Ground truth kinematic and geometric information from the original URDF files was processed and reorganized into a compact JSON format matching our model's output structure. The dataset is divided into standard training and testing sets. For detailed analysis based on object complexity, objects are further categorized into "simple" and "complex" subsets according to joint count and geometric intricacy. More details are reported in Appendix \ref{dataset_details}.

\textbf{Baselines:} 
We compare against three prior methods: (1)\textbf{Articulate-Anything,} an actor-critic system for iterative refinement via a mesh retrieval mechanism to generate code that can be compiled into simulators. (2) \textbf{Real2Code:} an approach that represents object parts with oriented bounding boxes, and uses a fine-tuned LLM to predict joint parameters as code. (3)\textbf{URDFormer:} a pipeline that constructs simulation scenes complete with articulated structure directly from real-world images.



\textbf{Evaluation Metrics:} \label{sec:evaluation_metrics}
We evaluate the performance of our URDF-Anything framework on three key aspects: part-level geometric segmentation, kinematic parameter prediction accuracy, and the physical executability of the final reconstructed URDF.
\begin{itemize}[leftmargin=*]
\item \textbf{Part Segmentation Accuracy:}
For evaluating how accurately our method segments the point cloud into individual links, we use mIoU.  A higher mIoU indicates better alignment between predicted and ground truth part geometry.

\item \textbf{Joint Parameter Prediction Accuracy:}
Following Articulate-Anything\cite{le2025articulateanything}, we evaluate the correctness of several critical components for each joint prediction compared to the ground truth URDF:
 (1)\textbf{Joint Type Error:} A binary metric indicating if the predicted joint type (e.g., revolute, prismatic) matches the ground truth.
 (2)\textbf{Joint Axis Error:} Quantifies the angular difference between the predicted and ground truth joint axes, normalized to be within $[0, \pi]$.
 (3)\textbf{Joint Origin Error:} Measures the positional error of the joint origin.
    % Optional: Add limit error if predicted and evaluated
    % \item \textbf{Joint Limit Error:} Evaluates the accuracy of predicted motion limits, comprising differences in motion range and direction.
A joint prediction is considered \textit{successful} only if the errors for all of its predicted components are within predefined small thresholds.

\item \textbf{Physical Executability:}
Beyond static accuracy metrics, the ultimate test of a reconstructed URDF is its functionality in a physics simulation. We evaluate the physical executability by loading the generated URDF models into a standard 3D simulator (e.g., Sapiens~\cite{khirodkar2024sapiens}). We then programmatically or manually attempt to actuate the joints. The physical executability metric is defined as the percentage of generated URDFs that can be loaded and actuated correctly in the simulator without exhibiting non-physical behavior (e.g., parts flying off, joints freezing, unexpected rotations/translations). This metric provides a crucial validation of the end-to-end reconstruction quality and its suitability for sim-to-real applications.

\end{itemize}


\subsection{Link Segmentation Results}
Table~\ref{tab:Segmentation Results} presents the quantitative results for part-level geometric segmentation. This evaluation assesses how accurately each method can delineate the individual links of an articulated object within its point cloud representation.  
% Figure\ref{fig:} provides visual examples of our link segmentation results on various object instances.
We compare our proposed method, denoted as URDF-Anything ($[SEG]$), against two baselines that represent different configurations of utilizing Uni3D features: Uni3D w/o text, which performs segmentation using only geometric features extracted by Uni3D, and Uni3D w/ text, which incorporates global text features alongside Uni3D features for segmentation, but without our dynamic $[SEG]$ token mechanism.  

Our method achieves state-of-the-art performance across all metrics and datasets (All, In-Distribution (ID), and Out-of-Distribution (OOD)). Quantitatively, URDF-Anything ($[SEG]$) significantly outperforms the best baseline on average, achieving 0.63 mIoU (a \textbf{16.7\%} improvement) and 0.97 Count Accuracy (a \textbf{15.4\%} improvement). This strong performance holds for both ID and OOD data, particularly on challenging OOD instances where our method achieves 0.62 mIoU and 0.96 Count Accuracy, demonstrating superior generalization capability compared to baselines.
The significant improvement in mIoU on out-of-distribution (OOD) data demonstrates superior generalization capability in segmenting novel object geometries and structures not seen during training. 
% Furthermore, the MLLM's inherent ability to process language instructions, combined with our dynamic $[SEG]$ token mechanism, proves particularly effective in accurately identifying and counting the correct number of parts for in-distribution objects, leveraging its internal representations and understanding. 


% \begin{minipage}{0.5\textwidth} % Allocate 60% of the text width for the first table
%   % \centering % Uncomment if you want the content of the minipage (the table) centered within the minipage
%   \begin{table}[H] % Using [H] from float package to place table here. Remove [H] if not desired/float package not used.
%         \caption{\textbf{Quantitative Results for Part-Level Link Segmentation.} Comparison of our method ({[}SEG{]}(Ours)) against baselines (uni3d w/o text, uni3d w/ text) on In-Distribution (ID) and Out-of-Distribution (OOD) object instances. }
%   % \vspace{.2cm} % Optional vertical space
%   % \centering % This would center the table within the minipage. Redundant if minipage itself is centered and table fills width.
%   % \footnotesize % Uncomment to make font size smaller for this table
%   % \setlength{\tabcolsep}{1.5mm} % Adjust column separation (default is 6pt)
%     \begin{tabular}{lcccc}
%     \toprule
%       \multirow{2}{*}{Models} & \multicolumn{2}{c}{mIoU $\uparrow$} & \multicolumn{2}{c}{Count Acc $\uparrow$} \\ \cmidrule(r){2-5}
%                               & ID & OOD & ID  & OOD \\ \midrule \midrule
%       uni3d w/o text  & 3.95  & 0.2514 & 2.32 &    1.351\\
%       uni3d w/ text   & 3.68   & 0.2537 & 2.69  & 1.024 \\
%       \midrule
%       \rowcolor[HTML]{ECF4FF}
%       \textbf{{[}SEG{]}(Ours)}  & \textbf{2.85}  & \textbf{0.2553} & \textbf{3.16}  & \textbf{0.784} \\
%     \bottomrule
%     \end{tabular}
%   \label{tab:Segmentation Results}
%   \end{table}
% \end{minipage}% <--- IMPORTANT: Add % here to avoid unwanted space if \hfill is on the next line
% \hfill % Add horizontal space between the two minipages (distributes space)
% % 或者使用固定的间距：%\hspace{0.02\textwidth} % Add fixed horizontal space e.g. 2% of text width
% \begin{minipage}{0.45\textwidth} % Adjusted width slightly to ensure it fits with \hfill and potential padding
%   % \centering
%   \begin{table}[H] % Using [H] from float package.
%     \caption{\textbf{Physical Executability Rate (\% $\uparrow$) across methods on In-Distribution (ID) and Out-of-Distribution (OOD) object instances.}}
%   % \centering
%   % \vspace{0.2cm}
%   % \setlength{\tabcolsep}{6pt} % Adjust column separation if needed
%     \begin{tabular}{lcc}
%     \toprule
%       \textbf{Method} & ID & OOD \\
%     \midrule
%       Real2Code Oracle  & ?\% & ?\% \\
%       URDFormer Oracle & ?\% & ?\% \\
%       Articulate-Anything  & ?\% & ?\% \\
%       \midrule
%       \textbf{URDF-Anything(Ours)} & \textbf{?\%} & \textbf{?\%} \\
%     \bottomrule
%     \end{tabular}
%   \label{tab:physical-executability}
%   % \vspace{-0.3cm} % Be cautious with negative vspace, it can cause overlaps.
%   \end{table}
% \end{minipage}













  % 可选：如果希望整个并排的结构有一个总标题，可以在这里添加
  % \caption{并排展示两个表格的结果}
  % \label{fig:combined_tables}
% \end{figure}

    % \begin{table}
    % % \centering % This centering is redundant if minipage has \centering
    % % \vspace{0.2cm}
    % % \setlength{\tabcolsep}{6pt} % Adjust column separation if needed
    % \begin{tabular}{lcc}
    % \toprule
    % \textbf{Method} & ID & OOD \\
    % % \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    % % & Simple & Complex & Simple & Complex \\
    % \midrule
    % Real2Code Oracle  & ?\% & ?\% \\
    % URDFormer Oracle & ?\% & ?\% \\
    % Articulate-Anything  & ?\% & ?\% \\
    % \midrule
    % \textbf{URDF-Anything(Ours)} & \textbf{?\%} & \textbf{?\%} \\
    % \bottomrule
    % \end{tabular}
    %     \caption{\textbf{Physical Executability Rate (\% $\uparrow$) across methods on Simple and Complex subsets.}}
    % \label{tab:physical-executability}
    % \vspace{-0.3cm} % This vspace might affect vertical alignment between the two tables
    % \end{table}

% \usepackage{tabularx}

\begin{table}[t] 
  \caption{\textbf{Quantitative Results for Part-Level Link Segmentation.} Comparison of our method ({[}SEG{]}(Ours)) against baselines (Uni3D w/o text, Uni3D w/ text) on In-Distribution (ID) and Out-of-Distribution (OOD) object instances. Performance is measured by mIoU (segment accuracy) and Count Accuracy (Count Acc), both where higher is better ($\uparrow$).}
  \vspace{.2cm}
  \centering
    \footnotesize
    \setlength{\tabcolsep}{1.5 mm}
    \begin{tabular}{lccccccc}
    \toprule
    \multirow{2}{*}{Models} & \multicolumn{3}{c}{mIoU $\uparrow$} & \multicolumn{3}{c}{Count Acc $\uparrow$} \\ \cmidrule(r){2-7} 
                            & ALL & ID & OOD & ALL & ID  & OOD \\ \midrule \midrule
     Uni3D w/o text  & 0.36 & 0.50 & 0.33 & 0.73 & 0.83 &   0.70\\
     Uni3D w/ text   & 0.54 & 0.64 & 0.51 & 0.84 & 0.91  & 0.82 \\
     \midrule
    \rowcolor[HTML]{ECF4FF} 
    \textbf{URDF-Anything ({[}SEG{]})} & \textbf{0.63}(16.7\%$\uparrow$) & \textbf{0.69}  & \textbf{0.62} & \textbf{0.97}(15.4\%$\uparrow$) & \textbf{0.99}  & \textbf{0.96} \\ 
    \bottomrule
    \end{tabular}
  \label{tab:Segmentation Results}
  \vspace{-0.3cm}
\end{table}


% \begin{table}[!t]
% \centering
% \caption{\textbf{Physical Executability Rate (\% $\uparrow$) across methods on Simple and Complex subsets.}}
% \vspace{0.2cm}
% \setlength{\tabcolsep}{6pt} % Adjust column separation if needed
% \begin{tabular}{lcccc}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{ID Classes} & \multicolumn{2}{c}{OOD Classes} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% & Simple & Complex & Simple & Complex \\
% \midrule
% Real2Code Oracle & ?\% & ?\% & ?\% & ?\% \\
% URDFormer Oracle & ?\% & ?\% & ?\% & ?\% \\
% Articulate-Anything & ?\% & ?\% & ?\% & ?\% \\
% \midrule
% \textbf{URDF-Anything(Ours)} & \textbf{?\%} & \textbf{?\%} & \textbf{?\%} & \textbf{?\%} \\
% \bottomrule
% \end{tabular}
% \label{tab:physical-executability}
% \vspace{-0.3cm}
% \end{table}

\begin{table}[!h]
\centering
% \vspace{-.6cm}
\caption{\textbf{Quantitative Comparison of Joint Parameter Prediction Accuracy.} This table presents the average prediction errors for joint Type (fraction of incorrect), Axis (radians), and Origin (meters) across different methods. Results are shown for All, In-Distribution (ID), and Out-of-Distribution (OOD) object classes. Lower values indicate better performance ($\downarrow$).} 
\vspace{.2cm}
\setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}}& \multicolumn{3}{c}{\textbf{All Classes}} & \multicolumn{3}{c}{\textbf{ID Classes}} & \multicolumn{3}{c}{\textbf{OOD Classes}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
 & Type $\downarrow$ & Axis $\downarrow$ & Origin $\downarrow$ & Type $\downarrow$ & Axis $\downarrow$ & Origin $\downarrow$ & Type $\downarrow$ & Axis $\downarrow$ & Origin $\downarrow$ \\
\midrule
Real2Code Oracle & \meanstd{0.537}{0.014} & \meanstd{1.006}{0.723} & \meanstd{0.294}{0.417} & \meanstd{0.410}{0.029} & \meanstd{1.164}{0.671} & \meanstd{0.344}{0.479} & \meanstd{0.576}{0.016} & \meanstd{0.937}{0.734} & \meanstd{0.272}{0.386} \\
URDFormer Oracle & \meanstd{0.556}{0.025} & \meanstd{0.374}{0.666} & \meanstd{0.581}{0.355} & \meanstd{0.418}{0.036} & \meanstd{0.208}{0.532} & \meanstd{0.609}{0.357} & \meanstd{0.679}{0.032} & \meanstd{0.643}{0.766} & \meanstd{0.513}{0.340} \\
Articulate-Anything & \meanstd{0.021}{0.003} & \meanstd{0.141}{0.441} & \meanstd{0.200}{0.380} & - & - & - & - & - & - \\
\midrule
\textbf{URDF-Anything (Ours)} & 
\textbf{\meanstd{0.008}{0.001}} & \textbf{\meanstd{0.132}{0.486}} & \textbf{\meanstd{0.164}{0.260}} & \textbf{\meanstd{0.007}{0.001}} & \textbf{\meanstd{0.121}{0.392}} & \textbf{\meanstd{0.130}{0.224}} & \textbf{\meanstd{0.009}{0.001}} & \textbf{\meanstd{0.136}{0.502}} & \textbf{\meanstd{0.173}{0.270}} \\
\bottomrule
\end{tabular}%
}
\vspace{-.3cm}
\label{tab:joint-prediction-comparison}
\end{table}


\subsection{Joint Parameter Prediction Results}

Table~\ref{tab:joint-prediction-comparison} presents the quantitative results for joint parameter prediction accuracy. We compare our proposed framework, \textbf{URDF-Anything (Ours)}, against several prior methods.
As shown in Table~\ref{tab:joint-prediction-comparison}, URDF-Anything demonstrates superior performance compared to baseline methods across all evaluated categories. Specifically, our method achieves notably lower Type, Axis, and Origin errors when evaluated on All Classes, ID Classes, and particularly on OOD Classes.
This indicates a significant improvement in accurately predicting kinematic parameters for articulated objects, including robust performance on object categories not seen during training (OOD instances).

This strong performance on complex and out-of-distribution articulated objects highlights the effectiveness of our MLLM-based end-to-end approach. The MLLM's inherent capabilities in understanding complex structures and generalizing from large-scale pretraining, combined with our method's joint reasoning of geometry and kinematics, enables more accurate parameter prediction in challenging, unseen scenarios compared to prior methods that may struggle with complexity or lack strong generalization priors.



% \begin{table}[!t]
% \centering
% \vspace{-.6cm}
% \caption{\textbf{Comparison of average joint prediction errors across methods on Simple and Complex subsets (lower is better).} Errors are reported for In-Distribution (ID) and Out-of-Distribution (OOD) object instances. `Type' shows the fraction of incorrect joint type predictions, `Axis' error is measured in radians, and `Origin' error in meters. 95\% confidence interval is included for classification error (joint type) and standard deviation for continuous errors (axis and origin).}
% \vspace{.2cm}
% \setlength{\tabcolsep}{3pt}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccccccc}
% \toprule
% & \multicolumn{6}{c}{\textbf{ID Classes}} & \multicolumn{6}{c}{\textbf{OOD Classes}} \\
% \cmidrule(lr){2-7} \cmidrule(lr){8-13}
% \textbf{Method} & \multicolumn{3}{c}{\textbf{Simple}} & \multicolumn{3}{c}{\textbf{Complex}} & \multicolumn{3}{c}{\textbf{Simple}} & \multicolumn{3}{c}{\textbf{Complex}} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
% & Type $\downarrow$ & Axis $\downarrow$ & Origin $\downarrow$ & Type $\downarrow$ & Axis $\downarrow$ & Origin $\downarrow$ & Type $\downarrow$ & Axis $\downarrow$ & Origin $\downarrow$ & Type $\downarrow$ & Axis $\downarrow$ & Origin $\downarrow$ \\
% \midrule
% Real2Code & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} \\ 

% URDFormer & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} \\  
% Articulate-Anything & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} \\ 
% ShapeLLM-7B & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} & \meanstd{?}{?} \\ 
% \midrule

% \textbf{URDF-Anything (Ours)} & \textbf{\meanstd{?}{?}} & \textbf{\meanstd{?}{?}} & \textbf{\meanstd{?}{?}} & \textbf{\meanstd{?}{?}} & \textbf{\meanstd{?}{?}} & \textbf{\meanstd{?}{?}} & \textbf{\meanstd{?}{?}} & \textbf{\meanstd{?}{?}} & \textbf{\meanstd{?}{?}} & \textbf{\meanstd{?}{?}} & \textbf{\meanstd{?}{?}} & \textbf{\meanstd{?}{?}} \\ 
% \bottomrule
% \end{tabular}
% }
% \vspace{-.3cm}
% \label{tab:joint-prediction-comparison}
% \end{table}



\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{figure/nips_baseline_1.pdf}
    \caption{\textbf{Qualitative Comparison of Articulated Object Reconstruction Results.} The top row displays the input image for various articulated object instances (each column represents a different object). We can find that baseline methods frequently struggle in predicting incorrect object types, generating distorted geometry, or exhibiting significant errors in link placement, leading to misaligned or incorrect structures. }
    \label{fig:results-qual}
    \vspace{-.2cm}
\end{figure}



\subsection{Physical Executability}

\begin{table}[!t]
\centering
\caption{\textbf{Physical Executability Rate (\% $\uparrow$) across methods on Simple and Complex subsets.}}
\vspace{0.2cm}
\setlength{\tabcolsep}{6pt} % Adjust column separation if needed
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{ALL} & \multicolumn{2}{c}{ID Classes} & \multicolumn{2}{c}{OOD Classes} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & Simple & Complex & Simple & Complex \\
\midrule
URDFormer Oracle & 24\%& 40\% & 23\% & 27\% & 11\% \\
Articulate-Anything & 52\%& 71\% & 42\% & 69\% & 35\% \\
\midrule
\textbf{URDF-Anything(Ours)} & \textbf{78\%}(50.0\%$\uparrow$) & \textbf{90\%} & \textbf{78\%} & \textbf{83\%} & \textbf{67\%} \\
\bottomrule
\end{tabular}
\label{tab:physical-executability}
\vspace{-0.3cm}
\end{table}

% \begin{table}[!t]
% \centering
% \caption{\textbf{Physical Executability Rate (\% $\uparrow$) across methods on Simple and Complex subsets.}}
% \vspace{0.2cm}
% \setlength{\tabcolsep}{6pt} % Adjust column separation if needed
% \begin{tabular}{lccccc}
% \toprule
% \textbf{Method} & ALL & \multicolumn{2}{c}{ID Classes} & \multicolumn{2}{c}{OOD Classes} \\

% & & Simple & Complex & Simple & Complex \\
% \midrule
% URDFormer Oracle & 40\%& 40\% & 23\% & 27\% & 11\% \\
% Articulate-Anything & 40\%& 71\% & 42\% & 71\% & 42\% \\
% \midrule
% \textbf{URDF-Anything(Ours)} & \textbf{90\%}(16.7\%$\uparrow$) & \textbf{90\%} & \textbf{78\%} & \textbf{83\%} & \textbf{67\%} \\
% \bottomrule
% \end{tabular}
% \label{tab:physical-executability}
% \vspace{-0.3cm}
% \end{table}



Beyond evaluating static link segmentation and joint parameter accuracy, a critical validation of our end-to-end reconstruction framework is the physical executability of the generated URDF models in a simulation environment. 
As defined in Section~\ref{sec:evaluation_metrics}, this metric assesses the percentage of generated URDFs that can be successfully loaded and actuated in a physics simulator without errors or non-physical behavior. 

As shown in Table~\ref{tab:physical-executability}, URDF-Anything achieves a high physical executability rate, significantly surpassing baseline methods, particularly for Complex and OOD objects. This demonstrates the superior overall pipeline robustness of our approach. Compared to prior methods like Real2Code~\cite{mandi2024real2code}, which rely on complex, sequential pipelines where errors in one step can cascade and require manual intervention for refinement, or Articulate-Anything~\cite{le2025articulateanything}, which may depend on iterative refinement  for parameter estimation, our framework utilizes a unified, end-to-end MLLM that jointly reasons about geometry and kinematics. This direct, integrated approach minimizes error propagation, allowing the model to leverage rich multimodal context for robust prediction of a consistent geometric and kinematic structure in a single pass. Figure \ref{fig:results-qual} and Figure\ref{fig:workflow} provides qualitative results illustrating the visual quality of our reconstructed articulated objects, showcasing both the generated link segmentation and the resulting mesh geometry for various challenging instances.




\subsection{Ablation Study}

\textbf{Impact of the geometric representation Modality.}
We conducted an ablation study to analyze the impact of input modalities on joint parameter prediction accuracy (Table~\ref{tab:ablation_joint_params}). 
Image-based variants include an off-the-shelf Image+Text MLLM ('Qwen2.5-VL-7B') and its fine-tuned version ('Qwen2.5-VL-7B + ft'), both utilizing 2D Image pixels and text prompts as input. It is evident that even these powerful state-of-the-art image MLLMs struggle to achieve the same level of accuracy in predicting precise 3D kinematic parameters compared to methods that leverage explicit 3D point cloud data. While fine-tuning ('Qwen2.5-VL-7B + ft') improves performance over the base image MLLM, the accuracy remains significantly lower than approaches starting from a 3D representation. This indicates that inferring precise 3D parameters solely from 2D images with current image MLLMs, without dedicated 3D processing, is highly challenging.

Furthermore, we analyze variants leveraging explicit 3D data. These include approaches using simplified geometry like 'OBB', which predicts parameters based on simplified Oriented Bounding Box representations, and variants using detailed point clouds. Among point cloud-based variants, we compare 'Point Cloud only', which relies solely on raw point cloud features without explicit text guidance, and our full method, 'Point Cloud + Text (Ours)', which processes detailed point cloud features integrated with text instructions using our 3D MLLM framework.
The 'OBB' variant demonstrates that simplified geometric representations are insufficient, as the loss of detail impacts parameter accuracy. The comparison between 'Point Cloud only' and 'Point Cloud + Text (Ours)' highlights the crucial role of text instructions in guiding the MLLM's 3D understanding and parameter prediction for this structured task.
Our full model, 'Point Cloud + Text (Ours)', which combines the rich geometric detail of point clouds with the reasoning and guidance power of language within a 3D MLLM framework, significantly outperforms all other variants. This ablation study validates that achieving high accuracy in articulated object parameter prediction requires both detailed 3D geometric input and effective language guidance processed by a model capable of joint multimodal and 3D spatial reasoning, supporting the design choices of our URDF-Anything framework.


\begin{table}[!t]
\centering
\caption{\textbf{Ablation Study on Input Modality for Joint Parameter Prediction.}}
\vspace{0.2cm}
\setlength{\tabcolsep}{8pt} % Adjust column separation if needed
\begin{tabular}{lcccc}
\toprule
\textbf{Method Variant} & Input Modality & Type $\downarrow$ & Axis $\downarrow$ & Origin $\downarrow$ \\
\midrule
OBB & Text & 0.42 & 0.70 & 0.47 \\ 
Point Cloud only & Point Cloud & 0.34 & 0.29 & 0.26 \\ 
Qwen2.5-VL-7B & Image + Text & 0.57 & 0.85 & 0.23 \\ 
Qwen2.5-VL-7B + ft & Image + Text & 0.38 & 0.81 & 0.18 \\ 
\midrule
\textbf{Point Cloud + Text (Ours)} & Point Cloud + Text & \textbf{0.008} & \textbf{0.132} & \textbf{0.164} \\
\bottomrule
\end{tabular}
\label{tab:ablation_joint_params}
\vspace{-0.3cm}
\end{table}

==> sec/5_Conclusion_and_Discussion.tex <==
\section{Conclusion} \label{Conclu}

In this paper, we presented \textbf{URDF-Anything}, a novel end-to-end framework that leverages the power of 3D Multimodal Large Language Models (MLLMs) to reconstruct functional URDF digital twins of articulated objects directly from visual observations. By utilizing the MLLM's inherent capabilities and introducing a dynamic $[SEG]$ token mechanism for joint geometric segmentation and kinematic parameter prediction, our method overcomes limitations of prior decoupled or simplified approaches. Experiments demonstrate that URDF-Anything achieves state-of-the-art performance across segmentation, parameter prediction, and physical executability metrics on the PartNet-Mobility dataset, exhibiting superior generalization to complex and unseen objects. This work provides a robust and efficient solution for automated articulated object digital twin creation, significantly advancing capabilities for robotic simulation.


\textbf{Limitations.} While URDF-Anything demonstrates significant advancements, limitations include the inability to generate certain URDF properties (e.g., mass, moment of inertia), partly due to training data and base model constraints. Additionally, the pipeline is not fully end-to-end, relying on an external point-to-mesh conversion module to generate link geometry. Precision of numerical parameters is also limited by the token-based generation approach.

\clearpage

==> sec/checklist.tex <==

\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit.

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA).
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize}


%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our contributions claimed correspond with experiment result in Section\ref{Exp} and we provide detailed figures and tables.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers.
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings.
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss limitations in Section\ref{Conclu}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper.
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This study focuses on empirical/applied aspects rather than theoretical derivations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results.
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition.
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced.
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide experiment detail in Section\ref{Exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable.
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide supplemental material, including instruction to download and prepare data and how to use our code and derive the result. We also include our code.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide experiment details in section\ref{Exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The reported experimental results are not accompanied by error bars, confidence intervals, or statistical significance tests to quantify the variability of the performance metrics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include compute resources information in section\ref{Exp}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute.
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper).
    \end{itemize}

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We went through the guidelines carefully and we are sure that our research conform, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper pose no such risks as a novel model.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper pose no such risks as a novel model.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters.
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cite all relevant papers in out references.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide detailed README file in supplementary material for ease of use.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc.
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We don't involve crowdsourcing and human subjects. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper.
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector.
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We don't involve crowdsourcing and human subjects. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution.
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The proposed framework utilizes a Large Language Model as a core and important component of its methodology. The role and implementation details of the LLM are described in Section \ref{MLLM} and Section \ref{Exp}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

